Reachable Sets of Classifiers and Regression Models: (Non-)Robustness Analysis and Robust Training

Neural networks achieve outstanding accuracy in classification and regression tasks. However, understanding their behavior still remains an open challenge that requires questions to be addressed on the robustness, explainability and reliability of predictions. We answer these questions by computing reachable sets of neural networks, i.e. sets of outputs resulting from continuous sets of inputs. We provide two efficient approaches that lead to over- and under-approximations of the reachable set. This principle is highly versatile, as we show. First, we use it to analyze and enhance the robustness properties of both classifiers and regression models. This is in contrast to existing works, which are mainly focused on classification. Specifically, we verify (non-)robustness, propose a robust training procedure, and show that our approach outperforms adversarial attacks as well as state-of-the-art methods of verifying classifiers for non-norm bound perturbations. Second, we provide techniques to distinguish between reliable and non-reliable predictions for unlabeled inputs, to quantify the influence of each feature on a prediction, and compute a feature ranking.

==> applications.tex <==
\section{Applications}
\label{sec:applications}

In the following we describe three different applications of our method for computing reachable sets. More specifically, we discuss (non-)robustness verification, quantification of feature importance and computing trust-indicators of predictions. All of them help us to explore and understand the predictions made by neural networks.

\subsection{(Non-)Robustness Verification}
\label{subsec:applications_robustness}

First, we evaluate the potential of reachable sets by using them for robustness/non-robustness verification of a classifier, i.e. for studying how predictions of a neural network change when perturbing input data instances. 
More precisely, we aim to understand how the predictions based on a certain input set behave (do they all map to the same class? do they vary?).
Formally, the set of predictions (class) is $P = \{\arg \max_c f(x)_c | x \in I\}$, given an input set $I$.

Traditionally, the input set is restricted to certain norm-balls around an anchor point.
Using zonotopes as input sets has the advantage that we can define very flexible perturbations for verification, formally specified by the generator matrix~$G$. 
The perturbed input sets can be cube-shaped, sets where each dimensions has a different extension and even complex sets that allow to analyze perturbations that couple input dimensions. 



\subsubsection{Robustness scores and Robust Training of Classifiers}
\label{subsubsec:robustness_scores}

For verification we compute a so called robustness score against each class. 
Let~$a$ be the label/predicted class, i.e. the one that corresponds to the highest logit for a specific input. 
Let $b \neq a$ denote the class against which we quantify robustness. The least robust point~$p$ within the reachable set (output/logit space)
is the one where its coordinate $p_b$ is very close to $p_a$ or even larger. Considering this, we define the robustness score against class~$b$ of reachable set $\{Z\}$ as: 
\begin{equation}
\begin{aligned}
	\mathrm{s}_b &= \min_{p, Z} \left(p_a - p_b \right) %
	             %
	              = \min_{Z} \left( c_a - c_b - \sum_i \left| g_i^a - g_i^b \right| \right) 
\end{aligned}
\label{eq:scores}
\end{equation}
where $p \in Z, Z \in \{Z\}$ and we use that $p_a = c_a + \sum_i \beta_i g_i^a$, $p_b = c_b + \sum_i \beta_i g_i^b$ and $\sum_i \beta_i (g_i^a - g_i^b)$ is minimal when~$\beta_i \in \{-1, 1\}$ depending on the sign of $g_i^a - g_i^b$. 

Robustness certificates are obtained by computing the scores against {all} classes $b\neq a$ on the \textit{over}-approximated reachable set $\{Z\}_O$. If \textit{all} scores are \textit{positive}, the robustness certificate holds: all points from the input set are classified as class $a$. Non-robustness certificates are obtained by checking if there is a class~$b$ such that $s_b$ on the \textit{under}-approximated reachable set $\{Z\}_U$ is \textit{negative}: at least one point from the input set is classified as class $b$.

These scores have four benefits: 
(i) They can be computed efficiently by simply iterating over all generators (see Equation~\ref{eq:scores}). 
(ii) The scores can be used for \textit{class specific verification} of robustness/ non-robustness (i.e. statements like: robust against class $b_1$, but non-robustness against class~$b_2$). 
(iii) The scores allow to quantify robustness/non-robustness relatively: A reachable set with a high score is more robust than one with a low score. 
(iv) Robustness scores can be used for robust training. To this end, we propose to following loss function: 


\begin{equation}
\begin{aligned}
L &= 
\begin{cases}
L_{\mathrm{pred}} + \max_b \mathrm{ReLU} \left( - s_b \right)  & \mathrm{if~prediction = target} \\
L_{\mathrm{pred}}                    & \mathrm{else} \\
\end{cases}
\end{aligned}
\label{eq:loss_classification}
\end{equation}
where the prediction loss describes a standard loss function used to train neural networks for classification (e.g. cross-entropy-loss). This combined loss function has the advantage that it minimizes the prediction loss for wrongly classified samples and considers the robustness loss for correctly classified ones. The term $\max_b \mathrm{ReLU} \left( - s_b \right)$, that captures robustness is zero for robust input sets, otherwise positive. 
These training function allows to train neural networks against any perturbation that can be described by an (input) zonotope. This involves standard perturbation like the $L_{\infty}$-norm around an input, a different perturbation on each input feature (axis-aligned parallelotope/box as input set) and complex perturbations that need to couple input features. Such a complex perturbation might be different brightness of picture, i.e. the simultaneous shift of all pixel values to a brighter/darker value. 













\subsection{Explainability: Feature Importance}
\label{subsec:applications_explain}

A second application of reachable sets is explaining predictions of a neural network. More precisely, reachable sets allow to quantify the importance of features regarding a classification decision. 

To quantify the importance of feature~$f_1$ for the prediction of~$x$, we define a box shaped input set~$\hat{Z}_{f_1} = (x | G)$ around~$x$ that allows a perturbation~$\delta$ on~$f_1$ but only a very small perturbation $\varepsilon$ on all other features. More formally, we use a diagonal input matrix~$G$, where~$G_{1,1} = \delta$ and~$G_{i,i} = \varepsilon~ \forall i \neq 1$. 
The larger the reachable set corresponding to~$\hat{Z}_{f_1}$, the higher the influence of feature~$f_1$ on the prediction. 

Thus, to quantify the importance of feature~$f_1$ we estimate the volume of the over-approximated reachable set. While in general, it is not efficient to compute the exact volume of a zonotope due to an exponential number of summands (see~\cite{gover2010}), computing the volume of the interval-hull of a zonotope is fast. Here, we use the scaled version of the volume that considers dimensionality~$d$ of the zonotope: 
$V \left(\mathrm{IH} (Z)\right) = \left( 2 \prod_i \delta g_i \right)^{\frac{1}{d}}$
where $\delta g$ is the same as in Equation~\ref{eq:interval_hull}.
The volume of the reachable set is estimated as the sum over all interval-hull volumes. 
















\subsection{Trust-Indicators of Predictions}
\label{subsec:applications_confidence}

As discussed before, an input is robust if the robustness score is positive against all other classes. Input sets with small scores are less robust than ones with high scores. 
Theoretically, a wrong prediction (w.r.t. ground truth) can be very robust. However, we have noticed that robustness scores corresponding to wrongly predicted inputs are often negative or close to zero.


Thus, we analyze $\theta$-robustness: Inputs are considered as $\theta$-robust if their scores are larger than some threshold~$\theta$.  We first compute robustness scores for the whole data-set (including wrongly predicted points). Then we compute the true-above-rate (TA) and the false-above-rate (FA) for different thresholds~$\theta$. These rates are related to true-positive-rate/false-positive rate used in receiver operating characteristic curves (ROC) and defined as follows: 
\begin{equation}
\begin{aligned}
	\mathrm{TA~rate} (\theta)  = \frac{N_{c, \theta}}{N_{c}}, \mathrm{~~and~~}
	\mathrm{FA~rate} (\theta)  = \frac{N_{w, \theta}}{N_{w}} 
\end{aligned}
\label{eq:ta_fa_rates}
\end{equation}
where $N_{c,\theta}$/ $N_{w, \theta}$ is the number of correctly/wrongly predicted points that is robust with respect to~$\theta$ and $N_c$ / $N_w$ the number of correctly/ wrongly predicted points. 
The best threshold~$\theta$ results in a high TA-rate indicating that most correctly classified points are $\theta$-robust/trustworthy, while the FA-rate should be low such that wrongly-classified points are not $\theta$-robust. 
The threshold~$\theta$ can be estimated by using the same setup as for ROC-curves, i.e.\ testing different thresholds on the train-set. 

Applying $\theta$-robustness verification allows to be more confident in a prediction if the label of an input is unknown (i.e. during the test phase; here we do not know the ground truth but we can evaluate $\theta$-robustness) and thus provides two properties: robustness and confidence. 







\subsection{Robustness Analysis and Robust Training for Regression Models}
\label{subsec:applications_regression}

Obtaining robust neural networks is desirable in any task, but has mainly been studied for classification. In classification tasks, an input~$x$ is robust if all points of its neighborhood are assigned the same label as~$x$. Thus, robustness is strongly based on decision boundaries. Regression tasks lack such a hard decision boundary, the output are not categorical, but continuous. However, intuitively we want that close inputs result in close outputs. 

To obtain an equal scale of all input features and outputs, we assume that the inputs and outputs of a neural network are standardized before training. Thus, a regression model follows this closeness property if the range of input features is the same as for output features. 

To analyze neural networks used for regression we compute the reachable set of the neural network (as described in \cite{kopetzki2020}). Based on this, we compute the range of each output value. Following the intuition that close input should result in close outputs the range of an output value and the range of an input feature should have the a similar size (if both are standardized). Thus, we compute the size of the ouput value range of output value~$a$ of the reachable set~$R_Z$:
\begin{equation}
\begin{aligned}
l_a &= \left| \max_{u \in R_Z}  u^a - \min_{v \in R_Z} v^a \right|
\end{aligned}
\label{eq:regression_output_range}
\end{equation}

If the size~$l_a$ of output value~$a$ is in the same range as the size of the input ranges, the neural network fulfills  the property that close inputs result in close outputs, and thus can be considered as ``robust''. 

For training we combine the robust loss with a standard loss function~$L_{\mathrm{val}}$ used for regression models (e.g. the Huber-loss): 
\begin{equation}
\begin{aligned}
L &= L_{\mathrm{val}} + \mathrm{ReLU} \left( \max_{a} l_a - l_{\mathrm{in}} \right)
\end{aligned}
\label{eq:regression_loss}
\end{equation}
where~$l_{\mathrm{in}}$ is the size of the range of input features. If $l_a$ is larger than~$l_{\mathrm{in}}$ then $L_{\mathrm{rob}}$ is positive, otherwise it is zero. Thus, training with this loss function results neural networks that map input sets on output sets such that the range of the output values is not larger than the range of the input features. 


\subsection{Analysis of Autoencoders}
\label{sec:analyze_autoencoder}



Reachable sets can be computed for any network, regardless of the application. However, the number of convex subset that define the reachable sets scales up exponentially for the proposed approach. To apply reachable set computation on autoencoders we modify the approach proposed in~\cite{kopetzki2020} such that the total number of convex subsets is $\leq B$ and the ``blow-up'', i.e. how many convex subset are generated to approximate~$\mathrm{ReLU} (Z)$ where~$Z$ is one zonotope is $\leq A$. 

The blow-up, i.e. the number of zonotopes resulting from applying ReLU on a zonotope~$Z = (c \mid G)$ can be estimated by the number quadrants that contain points of~$Z$. All point within one quadrant are either mapped on themselves or mapped to zero by ReLU. The approach proposed in~\cite{kopetzki2020} considers each subset located in one quadrant separately, and thus the blow-up of~$\mathrm{ReLU} (Z)$ is the number of quadrants in which~$Z$ is located. 

To estimate the number of quadrants~$q$, we first compute the interval-hull of~$Z$ (see \todo{..})
With respect to dimension~$d$, all points within~$Z$ are in the interval $\left[ l_{\mathrm{low}}^d, l_{\mathrm{upp}}^d = \right] \left[c_d - \delta g_d, c_d + \delta g_d \right]$. Next we count the number~$R_n$ of dimensions~$d$ where $l_{\mathrm{low}}^d < 0$ and $l_{\mathrm{upp}}^d > 0$.  The number of quadrants is $q = 2^{R_n}$. 
If $q > A$, we over-approximate~$\mathrm{ReLU} (Z)$ by computing it's interval-hull and restricting the intervals to the positive part. 


In case the number of zonotopes becomes larger than~$B$, we estimate the size of each zonotope, keep the largest~$B-1$ zonotopes and union the others over-approximatively. As size measure we use the extension of the interval-hull: 
\begin{equation}
\begin{aligned}
\mathrm{size}\left(Z\right) = \sum_d \log (\delta g)_d, ~~ \delta g = \sum_{i} |g_i|, 
\label{eq:size_measure}
\end{aligned}
\end{equation}
The over-approximative union of a set of zonotopes is computes by computing the interval-hull of each zonotope and minimizing/maximizing over the lower/upper limits of the interval-hull. The resulting interval is then transformed in the G-representaiton of a zonotope: 
\begin{equation}
\begin{aligned}
l_{\mathrm{low}}   &= \min_{Z_k} (c_k - (\delta g)_k), ~~  
l_{\mathrm{upp}}    = \max_{Z_k} (c_k + (\delta g)_k)     \\
Z_{\mathrm{uni}}   &= ( l_{\mathrm{low}} + g_{\mathrm{ext}} \mid \mathrm{diag} (g_{\mathrm{ext}})),~~ 
g_{\mathrm{ext}}    = 0.5 (l_{\mathrm{upp}} - l_{\mathrm{low}} )
\label{eq:union_over}
\end{aligned}
\end{equation}
where $\mathrm{diag} (g_{\mathrm{ext}})$ is a diagonal matrix. 
Under-approximations are obtained by dropping zonotopes, i.e. by considering only a subset of the quadrants and by keeping the~$B$ largest under-approximations and drop the others. 

The obtained reachable set of an autoencoder is a set instances with the same features as the input. To analyze the mapping, we compute the extension of the range of each feature (as described for regression models). 







==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelim}



\subsection{Zonotopes}

A $d$-dimensional zonotope~$Z$ is defined by the so called center~$c \in \mathbb{R}^d$ and a matrix~$G \in \mathbb{R}^{n \times d}$. Each row of~$G$ contains an $d$-dimensional vector~$g_i$, called generator. A zonotope~$Z$ is defined by the following set of points: 
\begin{equation}
\begin{aligned}
Z = (c \mid G) := \left\{ c + \sum_{i=1}^{n} \beta_i g_i \mid  \beta_i \in [-1,1] \right\}\subset \mathbb{R}^d. \label{eq:zonotope}
\end{aligned}
\end{equation}


\subsection{Reachable Sets of Feed-forward ReLU Neural Networks}


We use the approach proposed in~\cite{kopetzki2020} to compute the reachable set of a feed-forward ReLU neural network. The authors propose to define an input set by an arbitrary zonotope an propagate it layer-by-layer through the neural network. In each layer two operations have to be performed on the input set. First, we need to apply a linear transformation defined by weights~$W$ and bias~$b$ on the input set~$Z = (c \mid G)$ of the layer. This linear transformation can be computed exactly: 
$Z' = (W c + b \mid G W^T)$. 
Second, the ReLU activation function has to be applied on~$Z'$. ReLU maps a points~$x \in \mathcal{R}^D$ dimension-wise on the maximum of zero and itself: $\max \{ x, \vec{0} \}$. Applying ReLU on a zonotope can result in a non-convex set. Thus, the authors ``split'' zonotope~$Z$ in subsets~$S_i$, such that each subset is located in one quadrant, approximate each~$S_i$ by a zonotope~$Z_i$ and apply ReLU on~$Z_i$. If $Z_i$ is located in one quadrant, $\mathrm{ReLU} (Z_i)$ can be computed exactly. Thus, applying ReLU on~$Z'$ is approximated by a set of zonotopes. Each zonotope of the set if further propagate through the neural network and the output or reachable set of the neural network is approximated by a set of zonotopes. If the outcome of ReLU is over-approximated)in each layer we obtain an over-approximation of the reachable set, if we under-approximate in each layer an under-approximation. The details of these computations are described and discussed in~\cite{kopetzki2020}. 


The advantage of this technique is that reachable sets can be computed for any feed-forward ReLU network. However, as the number of zonotopes scales up with the size of the input set, the number of neurons and the number of layer it is only feasible for small/medium neural networks. 


==> references.tex <==
\section*{References}



==> theory.tex <==










==> theory_autoencoder.tex <==

\subsection{Analysis of Autoencoders}
\label{sec:analyze_autoencoder}



Reachable sets can be computed for any network, regardless of the application. However, the number of convex subset that define the reachable sets scales up exponentially for the proposed approach. To apply reachable set computation on autoencoders we modify the approach proposed in~\cite{kopetzki2020} such that the total number of convex subsets is $\leq B$ and the ``blow-up'', i.e. how many convex subset are generated to approximate~$\mathrm{ReLU} (Z)$ where~$Z$ is one zonotope is $\leq A$. 

The blow-up, i.e. the number of zonotopes resulting from applying ReLU on a zonotope~$Z = (c \mid G)$ can be estimated by the number quadrants that contain points of~$Z$. All point within one quadrant are either mapped on themselves or mapped to zero by ReLU. The approach proposed in~\cite{kopetzki2020} considers each subset located in one quadrant separately, and thus the blow-up of~$\mathrm{ReLU} (Z)$ is the number of quadrants in which~$Z$ is located. 

To estimate the number of quadrants~$q$, we first compute the interval-hull of~$Z$~\cite{kuehn1998}
\begin{equation}
\begin{aligned}
	\mathrm{IH}\left(Z\right) := \left[c - \delta g, c + \delta g \right], ~~ \delta g = \sum_{i} |g_i|, 
	\label{eq:interval_hull}
\end{aligned}
\end{equation}
where $\left|.\right|$ is the element-wise absolute value. With respect to dimension~$d$, all points within~$Z$ are in the interval $\left[ l_{\mathrm{low}}^d, l_{\mathrm{upp}}^d = \right] \left[c_d - \delta g_d, c_d + \delta g_d \right]$. Next we count the number~$R_n$ of dimensions~$d$ where $l_{\mathrm{low}}^d < 0$ and $l_{\mathrm{upp}}^d > 0$.  The number of quadrants is $q = 2^{R_n}$. 
If $q > A$, we over-approximate~$\mathrm{ReLU} (Z)$ by computing it's interval-hull and restricting the intervals to the positive part. 


In case the number of zonotopes becomes larger than~$B$, we estimate the size of each zonotope, keep the largest~$B-1$ zonotopes and union the others over-approximatively. As size measure we use the extension of the interval-hull: 
\begin{equation}
\begin{aligned}
	\mathrm{size}\left(Z\right) = \sum_d \log (\delta g)_d, ~~ \delta g = \sum_{i} |g_i|, 
	\label{eq:size_measure}
\end{aligned}
\end{equation}
The over-approximative union of a set of zonotopes is computes by computing the interval-hull of each zonotope and minimizing/maximizing over the lower/upper limits of the interval-hull. The resulting interval is then transformed in the G-representaiton of a zonotope: 
\begin{equation}
\begin{aligned}
	l_{\mathrm{low}}   &= \min_{Z_k} (c_k - (\delta g)_k), ~~  
	l_{\mathrm{upp}}    = \max_{Z_k} (c_k + (\delta g)_k)     \\
	Z_{\mathrm{uni}}   &= ( l_{\mathrm{low}} + g_{\mathrm{ext}} \mid \mathrm{diag} (g_{\mathrm{ext}})),~~ 
	g_{\mathrm{ext}}    = 0.5 (l_{\mathrm{upp}} - l_{\mathrm{low}} )
	\label{eq:union_over}
\end{aligned}
\end{equation}
where $\mathrm{diag} (g_{\mathrm{ext}})$ is a diagonal matrix. 
Under-approximations are obtained by dropping zonotopes, i.e. by considering only a subset of the quadrants and by keeping the~$B$ largest under-approximations and drop the others. 

The obtained reachable set of an autoencoder is a set instances with the same features as the input. To analyze the mapping, we compute the extension of the range of each feature (as described for regression models). 











==> theory_classification.tex <==
\section{Analysis and Robust Training of ReLU Networks}

\subsection{Robust Training of Classifiers}
\label{sec:train_classifiers}

A classifier is considered as robust if an input and its close neighborhood are assigned the same label. By computing the reachable set for perturbed input~$x$ of a neural network, we obtain information about the labels of the neighborhood of~$x$. 
This reachable label set is described by a set of zonotopes. 
We compute the least robust output point~$o^*$ and its correspnding robustness score~$s_{o^*}$ of the reachable set~$R_Z = \{Z_k\}_k$ as proposed in~\cite{kopetzki2020} (see Figure~\ref{fig:classification_train}). 
\begin{figure}[ht]
	\centering
	\begin{subfigure}{0.4\textwidth}
		\resizebox{!}{2cm}{\input{pics/z_reachset.tex}}
		\caption{Computation of reachble sets.}
		\label{fig:background_reachset}
	\end{subfigure}
	\hspace{0.5cm}
	\begin{subfigure}{0.2\textwidth}
		\resizebox{!}{2cm}{\input{pics/z_classification.tex}}
		\caption{Classification.}
		\label{fig:classification_train}
	\end{subfigure}
	\hspace{0.5cm}
	\begin{subfigure}{0.22\textwidth}
		\resizebox{!}{2cm}{\input{pics/z_regression.tex}}
		\caption{Regression.}
		\label{fig:regression_train}
	\end{subfigure}
	\caption{Computation of reachable sets (blue) and robust training.}
	\label{fig:theory_class_reg}
\end{figure}


The least robust output, is the one that minimizes the value corresponding to the true label~$a$ and maximizes the value corresponding to a label~$b \neq a$:  
\begin{equation}
	\begin{aligned}
	o^* &= \argmin_{b, ~o \in Z_k \in R_Z} \left(o_a - o_b \right) 
	= \argmin_{b, o \in Z_k \in R_Z} \left( c^k_a - c^k_b - \sum_i \left| g_i^{k,a} - g_i^{k,b} \right| \right).
	\end{aligned}
	\label{eq:scores_classification}
\end{equation}
where we use that $o_a = c^k_a + \sum_i \beta_i g_i^{k, a}$, $o_b = c^k_b + \sum_i \beta_i g_i^{k, b}$ and $\sum_i \beta_i (g_i^{k,a} - g_i^{k,b})$ is minimal when~$\beta_i \in \{-1, 1\}$ depending on the sign of $g_i^{k,b} - g_i^{k,b}$. 
The corresponding score $s_{o^*} = \left(o^*_a - o^*_b \right)$ quantifies robustness with respect to the least robust class~$b$. If the reachable set is over-approximated and this score~$s_{o^*}$ is positive, it does not exist a point corresponding to outputs in~$R_Z$ that is assigned a different label than~$a$ (see~\cite{kopetzki2020}). The larger~$s_{o^*}$, the larger the distance to a wrong label and the more robust is the classifier around~$x$. If the score is negative and the reachable set is under-approximated, it exists a point in the neighborhood of~$Z$ that is assigned a label~$b \neq a$. 

Based on over-approximated reachable sets and the score $s_{o^*}$, we define the following robustness term~$L_{\mathrm{rob}}$:
\begin{equation}
\begin{aligned}
	L_{\mathrm{rob}} &= \mathrm{ReLU} \left( - s_{o^*} \right) 
	                  = \mathrm{ReLU} \left( \min_{b, ~o \in Z_k \in R_Z} - \left(o_a - o_b \right) \right) 
\end{aligned}
\label{eq:rob_loss_class}
\end{equation}
This robustness loss is zero for robust input sets, because $s_{o^*}$ is positive for such sets and positive for non-robust reachable sets. 
Our overall loss function is a combination of prediction loss and robustness loss: 
\begin{equation}
	\begin{aligned}
		L &= 
			\begin{cases}
				L_{\mathrm{pred}} + L_{\mathrm{rob}} & \mathrm{if~prediction = target} \\
				L_{\mathrm{pred}}                    & \mathrm{else} \\
			\end{cases}
	\end{aligned}
	\label{eq:loss_classification}
\end{equation}
where the prediction loss describes a standard loss function used to train neural networks for classification (e.g. cross-entropy-loss). This combined loss function has the advantage that it minimizes the prediction loss for wrongly classified samples and considers the robustness loss for correctly classified ones. 

These training function allows to train neural networks against any perturbation that can be described by an (input) zonotope. This involves standard perturbation like the $L_{\infty}$-norm around an input, a different perturbation on each input feature (axis-aligned parallelotope/box as input set) and complex perturbations that need to couple input features. Such a complex perturbation might be different brightness of picture, i.e. the simultaneous shift of all pixel values to a brighter/darker value. 










==> theory_fin.tex <==



==> theory_regression.tex <==


\subsection{Analysis of Regression Models}
\label{sec:analyze_regression}


Obtaining robust neural networks is desirable in any task, but has mainly been studied for classification. In classification tasks, an input~$x$ is robust if all points of its neighborhood are assigned the same label as~$x$. Thus, robustness is strongly based on decision boundaries. Regression tasks lack such a hard decision boundary, the output are not categorical, but continuous. However, intuitively we want that close inputs result in close outputs. 

To obtain an equal scale of all input features and outputs, we assume that the inputs and outputs of a neural network are standardized before training. Thus, a regression model follows this closeness property if the range of input features is the same as for output features. 

To analyze neural networks used for regression we compute the reachable set of the neural network (as described in \cite{kopetzki2020}). Based on this, we compute the range of each output value. Following the intuition that close input should result in close outputs the range of an output value and the range of an input feature should have the a similar size (if both are standardized). Thus, we compute the size of the ouput value range of output value~$a$ of the reachable set~$R_Z$:
 \begin{equation}
 \begin{aligned}
		l_a &= \left| \max_{u \in R_Z}  u^a - \min_{v \in R_Z} v^a \right|
 \end{aligned}
 \label{eq:regression_output_range}
 \end{equation}

If the size~$l_a$ of output value~$a$ is in the same range as the size of the input ranges, the neural network fulfills  the property that close inputs result in close outputs, and thus can be considered as ``robust''. 



\subsection{Robust Training of Regression Models}
\label{sec:train_regression}

Considering the robustness property defined above for regression models, we define the following robustness term for regression models:
 \begin{equation}
\begin{aligned}
	L_{\mathrm{rob}} &= \mathrm{ReLU} \left( \max_{a} l_a - l_{\mathrm{in}} \right)
\end{aligned}
\label{eq:regression_robust_loss}
\end{equation}
where~$l_{\mathrm{in}}$ is the size of the range of input features. If $l_a$ is larger than~$l_{\mathrm{in}}$ then $L_{\mathrm{rob}}$ is positive, otherwise it is zero. Thus, training with this loss function results neural networks that map input sets on output sets such that the range of the output values is not larger than the range of the input features. 
For training we combine the robust loss with a standard loss function~$L_{\mathrm{val}}$ used for regression models (e.g. the Huber-loss): 
 \begin{equation}
\begin{aligned}
	L &= L_{\mathrm{val}} + L_{\mathrm{rob}}
\end{aligned}
\label{eq:regression_loss}
\end{equation}



